Real-time Deep Learning at the Edge for Scalable Reliability Modeling of Si-MOSFET Power Electronics Converters

With the significant growth of advanced high-frequency power converters, on-line monitoring and active reliability assessment of power electronic devices are extremely crucial. This article presents a transformative approach, named Deep Learning Reliability Awareness of Converters at the Edge (Deep RACE), for real-time reliability modeling and prediction of high-frequency MOSFET power electronic converters. Deep RACE offers a holistic solution which comprises algorithm advances, and full system integration (from the cloud down to the edge node) to create a near real-time reliability awareness. On the algorithm side, this paper proposes a deep learning algorithmic solution based on stacked LSTM for collective reliability training and inference across collective MOSFET converters based on device resistance changes. Deep RACE also proposes an integrative edge-to-cloud solution to offer a scalable decentralized devices-specific reliability monitoring, awareness, and modeling. The MOSFET convertors are IoT devices which have been empowered with edge real-time deep learning processing capabilities. The proposed Deep RACE solution has been prototyped and implemented through learning from MOSFET data set provided by NASA. Our experimental results show an average miss prediction of $8.9\%$ over five different devices which is a much higher accuracy compared to well-known classical approaches (Kalman Filter, and Particle Filter). Deep RACE only requires $26ms$ processing time and $1.87W$ computing power on Edge IoT device.

==> biography.tex <==


\vspace{-2cm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./Fig/Bio/baharani}}]{Mohammadreza Baharani}
(S’18)
received the M.Sc. degree in computer engineering
from University of Tehran, Iran, in 2012. He is currently a graduate research assistant and  Ph.D. student in the TeCSAR group at the Department of Electrical and Computer Engineering, University of North Carolina at Charlotte, USA. His research goal is to solve real problems related to the intersection of computer architecture engineering and machine learning, in particular, hardware modeling of deep machine learning algorithms such as convolutional and recurrent neural networks, performance improvement of single-threaded general purpose processors based on open-source ISA, and efficiency improvement of hardware accelerator for compute-intensive algorithms with the aid of reconfigurable hardware architectures.
\end{IEEEbiography}

% if you will not have a photo at all:

\vspace{-2cm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./Fig/Bio/Mehrdad_Biglarbegian}}]{Mehrdad Biglarbegian}
(S’14) received
the B.S. degree in electrical
engineering the University of Tehran,
Iran, in 2010, the M.Sc. degree in energy
engineering from Politecnico di Milano,
Italy in 2014, and the Ph.D. degree in
electrical engineering from the University
of North Carolina at Charlotte, USA, in
2018. He is now a senior design for reliability engineer at Tesla,
Palo Alto, CA, USA. His expertise includes reliability
enhancement in power converters, high frequency wide
bandgap in power electronics applications, and advanced
sensing analysis of high frequency systems.
\end{IEEEbiography}


\vspace{-2cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./Fig/Bio/Babak_Parkhideh}}]{Babak Parkhideh}
(S’07–M’13–SM’16) received the B.Sc. (Hons.) degree from the University of Tehran, Tehran, Iran, in 2003, the M.Sc. degree from RWTH-Aachen University, Germany, in 2006, and the Ph.D. degree from North Carolina State University, USA, in 2012, all in electrical engineering. 
He is currently an Associate Professor in the Department of Electrical and Computer Engineering, University of North Carolina at Charlotte, USA, where he is also a Faculty Associate with the Energy Production and Infrastructure Center (EPIC) and the Founding Director of the PV Integration Laboratory (PIL). His research interests include PV/battery power electronic systems, high-frequency power converters, and high-bandwidth current-sensing schemes.
\end{IEEEbiography}

\vspace{-2cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./Fig/Bio/tabkhi_hamed}}]{Hamed Tabkhi}
(S’07–M’14) 
is an Assistant Professor in the Department of Electrical and Computer Engineering, University of North Carolina at Charlotte (UNC Charlotte), USA. He received his Ph.D. degree in 2014 from Northeastern University and was a post-doctoral research associate at Northeastern University till 2016. He is the founder and Principal Investigator (PI) of Transformative Computer Systems and Architecture Research Labs (TeCSAR) at UNC Charlotte. His research spans across entire computer stack from algorithm design to system software, edge computing, and microarchitecture. He focuses on novel transformative solutions to bring real-time edge intelligence to enable a broad range of smart cities applications, as well as understanding and modeling of complex physical and engineering systems.
\end{IEEEbiography}



%%%%%%%%%%% draft.bib %%%%%%%%%%%%%%%%%%%



% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks




